AdS/CFT Duality User Guide

This is the draft/updated version of a textbook on "real-world" applications of the AdS/CFT duality for beginning graduate students in particle physics and for researchers in the other fields. The aim of this book is to provide background materials such as string theory, general relativity, nuclear physics, nonequilibrium physics, and condensed-matter physics as well as some key applications of the AdS/CFT duality in a single textbook. Contents: (1) Introduction, (2) General relativity and black holes, (3) Black holes and thermodynamics, (4) Strong interaction and gauge theories, (5) The road to AdS/CFT, (6) The AdS spacetime, (7) AdS/CFT - equilibrium, (8) AdS/CFT - adding probes, (9) Basics of nonequilibrium physics, (10) AdS/CFT - nonequilibrium, (11) Other AdS spacetimes, (12) Applications to quark-gluon plasma, (13) Basics of phase transition, (14) AdS/CFT - phase transition, (15) Exercises.

==> Chap_others_app.tex <==
%\documentclass[11pt]{jarticle} %%% アンコメント
\ifx\nameofpaper\undefined %%% もし main.tex が読まれていなければ
  \usepackage{macro_natsuume} %%% 自分用のマクロファイルを読み込み，
  \def\beginsection{\section*}
  \def\endofsection{\end{document}} %%% \endofsection = \bye と定義
  \input draft_header.tex
\else %%% そうでなければ
  \def\beginsection{\chapter}
  \def\endofsection{\endinput} %%% \endofsection = \endinput と定義
\fi


%%%%%%%%%
\section{Appendix: Explicit form of other AdS spacetimes \advanced
%そのほかの時空の詳細（10章）
}\label{sec:others_details}
%%%%%%%%%

%%------------------
\subsection{SAdS$_{p+2}$ black hole}\label{sec:SAdSp+2}
%%------------------

In this section, we consider black holes with planar horizon only. 
The SAdS$_{p+2}$ black hole is given by
%$(p+2)$次元のシュワルツシルドAdSブラックホール（プラナー・ホライズン）は
%\begin{align}
%
%\action &= \frac{1}{16\pi G_{p+2}} \int d^{p+2}x\, \sqrt{-g} \left( R -2 \Lambda \right)~, \\
%2\Lambda &= - \frac{p(p+1)}{L^2}~.
%\label{eq:}
%
%\end{align}
%の解であり，
\begin{align}
%
ds_{p+2}^2 &= - f dt^2  + \frac{dr^2}{f} + \left(\frac{r}{L}\right)^2 d\bmx_{p}^2~, \\
f &= \left(\frac{r}{L}\right)^2 \left\{ 1 - \left( \frac{r_0}{r} \right)^{p+1} \right\}~.
%\label{eq:}
%
\end{align}
Thermodynamic quantities are given by
%熱力学量は，
%\begin{subequations}
%\label{eq:}
\begin{align}
%
T %= \frac{f'(r_0)}{4\pi} 
&= \frac{p+1}{4\pi L^2} r_0~,
\\ %\label{eq:}
s %= \frac{a}{4G}
&= \frac{1}{4 G_{p+2}} \left(\frac{r_0}{L}\right)^{p}~,
\\ %\label{eq:}
\varepsilon &= \frac{p}{16\pi G_{p+2} L} \left( \frac{r_0}{L} \right)^{p+1}~,
\\ %\label{eq:}
P &= \frac{1}{16\pi G_{p+2} L} \left( \frac{r_0}{L} \right)^{p+1} = \frac{1}{p}\varepsilon~.
%\label{eq:}
%
\end{align}
%\end{subequations}


%%-------------------------------------
\subsection{M-branes}\label{sec:M_brane}
%%-------------------------------------

%%-------------------------------------
\subsubsection*{Zero-temperature case}%\label{sec:}
%%-------------------------------------

The M2-brane at zero temperature is given by
%M2ブレーンは
\begin{align}
%
ds_{11}^2 &= f_2^{-2/3} (-dt^2 + dx_1^2 + dx_2^2) 
	+ f_2^{1/3} (dr^2 + r^2 d\Omega_{7}^2)~, \\
%A_{012} &=& f_2^{-1}, \\
f_2 &= 1+\left(\frac{r_2}{r}\right)^{6}.
\label{eq:M2}
%
\end{align}
In the near-horizon limit $r \ll r_2$, the metric becomes
%\sect{D3_brane}と同様，$r \ll r_2$ のnear-horizon極限では
\begin{align}
%
ds_{11}^2 &\rightarrow \left( \frac{r}{r_2} \right)^4 (-dt^2 + dx_1^2 + dx_2^2) 
	+ \left( \frac{r_2}{r} \right)^2 (dr^2 + r^2 d\Omega_{7}^2) \\
&= \left( \frac{2\tilr}{r_2} \right)^2 (-dt^2 + dx_1^2 + dx_2^2) 
	+ \left( \frac{r_2}{2} \right)^2 \frac{d\tilr^2}{\tilr^2} + r_2^2 d\Omega_{7}^2~,
%\label{eq:}
%
\end{align}
where $r =(2\tilr r_2)^{1/2}$. The geometry reduces to the AdS$_4 \times S^7$ spacetime with AdS radius $L = r_2/2$ and the $S^7$ radius $L_{S^7} = 2L = r_2$. Note that the AdS radius differs from the sphere radius unlike the D3-brane case.
%$r =(2\tilr r_2)^{1/2}$ とした．AdS半径 $L = r_2/2$ の AdS$_4 \times S^7$ に帰着する．ただしD3ブレーンとは異なり， $S^7$の半径$L_{S^7}$は$L_{S^7} = 2L = r_2$ で与えられる．

The M5-brane at zero temperature is given by
%M5ブレーンは
\begin{align}
%
ds_{11}^2 &= f_5^{-1/3} (-dt^2 + d\bmx_5^2) 
	+ f_5^{2/3} (dr^2 + r^2 d\Omega_{4}^2)~, \\
%A_{01 \cdots 6} &=& f_5^{-1}, \\
f_5 &= 1+\left(\frac{r_5}{r}\right)^{3}.
\label{eq:M5}
%
\end{align}
In the near-horizon limit $r \ll r_5$, the metric becomes
%near-horizon極限では
\begin{align}
%
ds_{11}^2 &\rightarrow \left( \frac{r}{r_5} \right) (-dt^2 + d\bmx_5^2) 
	+ \left( \frac{r_5}{r} \right)^2 (dr^2 + r^2 d\Omega_{4}^2) \\
&= \left( \frac{\tilr}{2r_5} \right)^2 (-dt^2 + d\bmx_5^2) 
	+ (2r_5)^2 \frac{d\tilr^2}{\tilr^2} + r_5^2 d\Omega_{4}^2~,
%\label{eq:}
%
\end{align}
% corrected: 2013/9/12
where $r = \tilr^2/(4r_5)$. The geometry reduces to the AdS$_7 \times S^4$ spacetime with AdS radius $L = 2r_5$ and the $S^4$ radius $L_{S^4} = L/2 = r_5$.
%$r = \tilr^2/(2r_5)$ とした．AdS半径 $L = 2r_5$ の AdS$_7 \times S^4$ に帰着する．ただし $S^4$の半径$L_{S^4}$は$L_{S^4} = L/2 = r_5$で与えられる．

%%-------------------------------------
\subsubsection*{AdS/CFT dictionary}%\label{sec:}
%%-------------------------------------

One can obtain the AdS/CFT dictionary for M-branes as in the D3-brane in \sect{D3_brane}. For the M2-brane, the number of the spatial dimensions transverse to the brane is eight. Thus, the Newtonian potential is  $G_{11}\tension_2/r^6$ instead of $GM/r$ in three spatial dimensions. Using the dimensional analysis and the fact that there are $N_c$ branes, one gets
%MブレーンのAdS/CFT辞書の作り方は，\sect{D3_brane}のD3の場合と同様である．M2の場合，ブレーンに垂直な空間次元は8である．したがって，ニュートン・ポテンシャルは空間3次元の $GM/r$ のかわりに， $G_{11}\tension_2/r^6$ となる．次元解析と$N_c$枚のブレーンがあることから，
\begin{align}
%
r_2^6 &\simeq G_{11}\tension_2 \simeq N_c l_{11}^6~, 
\label{eq:Newton_M2} \\
G_{11} &=: l_{11}^9~,
\label{eq:Planck11}
%
\end{align}
where $l_{11}$ is the 11-dimensional Planck length. In string theory, there is the fundamental length scale, the string scale $l_s$, and the Planck length $l_{10}$ is not fundamental. They are related to each other by $l_{10}^8 \simeq g_s^2 l_s^8$. However, in the 11-dimensions, it is not yet clear if there is a fundamental length scale like $l_s$, so here we use $l_{11}$ instead. From Eqs.~\eqref{eq:Newton_M2} and \eqref{eq:Planck11}, we get
%ここで $l_{11}$ は11次元プランク長さである．超弦理論では，ストリング長さ $l_s$ という基礎的なスケールがあり，プランク長さ $l_{10}$ は $l_s$ で $l_{10}^8 \simeq g_s^2 l_s^8$ と与えられる．しかし，11次元の場合，$l_s$ に相当するスケールがあるか不明なので，$l_{11}$ を使う．これらの関係から，
\be
%
\frac{r_2^9}{G_{11}} \simeq N_c^{3/2}~.
\label{eq:dictionary_M2}
%
\ee
This is the M2 version of the first equation of \eq{dictionary}.
%これはD3の場合，\eq{dictionary}の第1式に相当する式である．

For the M5-brane, the number of the spatial dimensions transverse to the brane is five. Thus, the Newtonian potential is  $G_{11}\tension_5/r^3$, so 
%M5ブレーンの場合，ブレーンに垂直な空間次元は5である．したがって，ニュートン・ポテンシャルは $G_{11}\tension_5/r^3$ となり，
\be
%
r_5^3 \simeq G_{11}\tension_5 \simeq N_c l_{11}^3~.
%\label{eq:}
%
\ee
Thus,
%したがって，
\be
%
\frac{r_5^9}{G_{11}} \simeq N_c^{3}~.
\label{eq:dictionary_M5}
%
\ee

If one works out numerical coefficients, the results are
%式~(\ref{eq:dictionary_M2}), (\ref{eq:dictionary_M5}) を係数まで注意してまとめたものは，
% corrected: 2013/12/10
\begin{alignat}{2}
%
N_c^{3/2} &= \frac{\sqrt{2} \pi^5 (2L)^9}{16\pi G_{11}}
= 12\sqrt{2} \pi \frac{L^2}{16\pi G_{4}}
&\quad& (\text{M2})~, 
\\
N_c^3 &= \frac{\pi^5L^9}{2\cdot16\pi G_{11}} 
= 3\pi^3\frac{L^5}{16\pi G_{7}}
&\quad& (\text{M5})~.
%\label{eq:}
%
\end{alignat}


%%-------------------------------------
\subsubsection*{Finite-temperature case}%\label{sec:}
%%-------------------------------------

The M2-brane at finite temperature is given by
%有限温度の場合，M2ブレーンは
\begin{align}
%
ds_{11}^2 &= f_2^{-2/3} (-hdt^2 + dx_1^2 + dx_2^2) 
	+ f_2^{1/3} (h^{-1}dr^2 + r^2 d\Omega_{7}^2)~, \\
h &= 1-\left(\frac{r_0}{r}\right)^{6} = 1-\left(\frac{\tilr_0}{\tilr}\right)^{3}~,
\label{eq:M2_non_extreme}
%
\end{align}
% corrected: 2013/9/13 
where $r_0 =(2\tilr_0 r_2)^{1/2}$. The M5-brane at finite temperature is given by
%M5ブレーンは，
\begin{align}
%
ds_{11}^2 &= f_5^{-1/3} (-hdt^2 + d\bmx_5^2) 
	+ f_5^{2/3} (h^{-1}dr^2 + r^2 d\Omega_{4}^2)~, \\
h &= 1-\left(\frac{r_0}{r}\right)^{3} = 1-\left(\frac{\tilr_0}{\tilr}\right)^{6}~,
\label{eq:M5_non_extreme}
%
\end{align}
% corrected: 2013/9/13 
where $r_0 = \tilr_0^2/(4r_5)$. In the near-horizon limit $\tilr_0 < \tilr \ll L$, the M2 and M5-branes reduce to the SAdS$_4$ and SAdS$_7$ black holes. One can then use the results of thermodynamic quantities for the SAdS$_{p+2}$ black hole. For example, the energy density for the M2-brane is given by
%$\tilr_0 < \tilr \ll L$の near-horizon 極限で，M2, M5はそれぞれ SAdS$_4$, SAdS$_7$ブラックホールに帰着する．熱力学量は，シュワルツシルドAdSブラックホールの結果（\sect{SAdSp+2}）をそのまま用いればよい．
\be
%
\varepsilon 
\simeq \frac{1}{G_4 L} \left( \frac{r_0}{L} \right)^{3}
\simeq \frac{L^9}{G_{11}} \left( \frac{r_0}{L^2} \right)^{3}
\simeq N_c^{3/2} T^3~,
%\label{eq:}
%
\ee
where $1/G_4 \simeq L^7/G_{11}$. For the M5-brane, 
\be
%
\varepsilon 
\simeq \frac{1}{G_7 L} \left( \frac{r_0}{L} \right)^{6}
\simeq \frac{L^9}{G_{11}} \left( \frac{r_0}{L^2} \right)^{6}
\simeq N_c^3 T^6~,
%\label{eq:}
%
\ee
where $1/G_7 \simeq L^4/G_{11}$. If one works out numerical coefficients, the results are 
%M2ブレーンの場合，
\begin{align}
%
s &= \sqrt{2} \pi^2 \left(\frac{2}{3}\right)^3 N_c^{3/2} T^2~, \\
\varepsilon &= \sqrt{2} \pi^2 \left(\frac{2}{3}\right)^4 N_c^{3/2} T^3~,
%\label{eq:}
%
\end{align}
for the M2-brane, and 
%M5ブレーンの場合，
% corrected: 2013/12/10
\begin{align}
%
s &= 3\pi^3 \left(\frac{2}{3}\right)^7 N_c^{3} T^5~, \\
\varepsilon &= \frac{5\pi^3}{2} \left(\frac{2}{3}\right)^7 N_c^{3} T^6~,
%\label{eq:}
%
\end{align}
for the M5-brane.

%%-------------------------------------
\subsection{D$p$-brane}\label{sec:Dp_brane}
%%-------------------------------------

%%-------------------------------------
\subsubsection*{Zero-temperature case}%\label{sec:}
%%-------------------------------------

The D$p$-brane at zero temperature is given by
%D$p$ブレーンは
%\begin{subequations}
%\label{eq:Dp_extreme}
\begin{align}
%
ds_{10}^2 &= Z_p^{-1/2} (-dt^2 + d\bmx_p^2) 
	+ Z_p^{1/2} (dr^2 + r^2 d\Omega_{8-p}^2)~, \\
e^{-2\phi} &= Z_p^{(p-3)/2}, \\
%A_{p} &= \frac{1}{g_s}(Z_p^{-1}-1) dx^0 \wedge dx^1 \wedge \cdots \wedge dx^p, \\
Z_p &= 1+ \left( \frac{r_p}{r} \right)^{7-p}.
%r_p^{7-p} &= \frac{(2\pi)^{7-p}}{(7-p) \Omega_{8-p}} g Q_p l_s^{7-p},
%
\end{align}
%\end{subequations}
When $p\neq3$, the dilaton $\phi$ has a nontrivial behavior.
%$p\neq3$ のとき，ディラトン $\phi$ がノントリビアルな振るまいをする．$p=3$ では，ディラトンは定数なのでこれまで考慮してこなかった．
In the near-horizon limit $r \ll r_p$, the metric becomes
%near-horizon 極限では，
\begin{align}
%
ds_{10}^2 &\rightarrow 
\left(\frac{r}{r_p}\right)^{(7-p)/2} ( -dt^2 + d\bmx_p^2 ) 
+ \frac{dr^2}{(\frac{r}{r_p})^{(7-p)/2}} 
+ r_p^2 \left(\frac{r}{r_p} \right)^{(p-3)/2} d\Omega_{8-p}^2
\label{eq:Dp_near_horizon1} \\
&= \left(\frac{r}{r_p}\right)^{(p-3)/2} \left\{ \left(\frac{r}{r_p}\right)^{5-p} ( - dt^2 + d\bmx_p^2 ) 
+ \frac{dr^2}{(\frac{r}{r_p})^2} 
+ r_p^2 d\Omega_{8-p}^2 \right\}~.
%
\end{align}
The metric is invariant up to an overall coefficient under a scaling:
\be
%
x^\mu \rightarrow a x^\mu~, \quad
r \rightarrow a^{-2/(5-p)} r~, \quad
ds^2 \rightarrow a^{-(p-3)/(5-p)} ds^2~.
%\label{eq:}
%
\ee

%%-------------------------------------
\subsubsection*{AdS/CFT dictionary}%\label{sec:}
%%-------------------------------------

One can obtain the AdS/CFT dictionary for the D$p$-branes as in the D3-brane in \sect{D3_brane}. For the D$p$-brane, the number of the spatial dimensions transverse to the brane is $(9-p)$. Thus, the Newtonian potential is $G_{10}\tension_p/r^{7-p}$. One thus obtains
%\begin{subequations}
%\label{eq:}
\begin{align}
%
r_p^{7-p} &\simeq g_s N_c l_s^{7-p}~, \\
G_{10} &\simeq g_s^2 l_s^8~, \\
g_s\, l_s^{p-3} &\simeq g_\text{YM}^2~,
%\label{eq:}
%
\end{align}
%\end{subequations}
where the last two expressions are Eqs.~\eqref{eq:string_vs_qft}. If one works out numerical coefficients, the results are
%\sect{D3_brane}のD3の場合と同様である．係数まで注意してまとめたものは，
%\begin{subequations}
% for Springer
%\label{eq:dictionary_Dp}
\begin{align}
%
r_p^{7-p} &= \frac{(2\pi)^{7-p}}{(7-p) \Omega_{8-p}} g_s N_c l_s^{7-p}~,
\label{eq:dictionary_Dp1} \\
16\pi G_{10} &= (2\pi)^7 g_s^2 l_s^8~, 
\label{eq:dictionary_Dp2} \\
2(2\pi)^{p-2}\, g_s\, l_s^{p-3} &= g_\text{YM}^2~.
\label{eq:dictionary_Dp3} 
%\label{eq:}
%
\end{align}
%\end{subequations}
When $p=3$, Eqs.~\eqref{eq:dictionary_Dp1}-\eqref{eq:dictionary_Dp3}  
%\eqref{eq:dictionary_Dp} 
reduces to Eqs.~\eqref{eq:dictionary} for the D3-brane.
%$p=3$ のとき，式~(\ref{eq:dictionary_Dp1})-(\ref{eq:dictionary_Dp3}) はD3ブレーンの場合の\eq{dictionary} に帰着する．また，\eq{dictionary_Dp3} の$l_s$ 依存性は，$(p+1)$次元のゲージ理論では $g_\text{YM}$ が次元をもつことを反映している．

%%-------------------------------------
\subsubsection*{Finite-temperature case}%\label{sec:}
%%-------------------------------------

The D$p$-brane at finite temperature is given by
%有限温度では，
\begin{align}
%
ds_{10}^2 &= Z_p^{-1/2} (-h dt^2 + d\bmx_p^2) 
%\nonumber \\
%	& &	\qquad\qquad 
+ Z_p^{1/2} (h^{-1}dr^2 + r^2 d\Omega_{8-p}^2)~, \\
%A_{p} &=& \coth\beta(f_p^{-1}-1) dx^0 \wedge dx^1 \wedge \cdots \wedge dx^p.
%Z_p &=& 1+\left(\frac{r_p}{r}\right)^{7-p}, \\
%= 1+(\frac{r_0}{r})^{d-p-3} \sinh^2\beta
h &= 1-\left(\frac{r_0}{r}\right)^{7-p}~,
%\label{eq:}
%
\end{align}
(in the so-called string metric). Thermodynamic quantities in the near-horizon limit are given by
%near-horizon極限での熱力学量は，
%\begin{subequations}
%\label{eq:}
\begin{align}
%
T %= \frac{f'(r_0)}{4\pi} =
&= \frac{7-p}{4\pi}\frac{r_0^{(5-p)/2}}{r_p^{(7-p)/2}}~,
\\ %\label{eq:}
s &= e^{-2\phi} \frac{a}{4G_{10}}
= \frac{1}{4 G_{10}} \Omega_{8-p} (r_p r_0)^{(7-p)/2} r_0~,
\\ %\label{eq:}
\varepsilon &= \frac{9-p}{32\pi G_{10}} \Omega_{8-p} r_0^{7-p}~,
\\ %\label{eq:}
% corrected: 2013/9/13
P &= \frac{5-p}{9-p} \varepsilon~,
\\ %\label{eq:}
C &:= \frac{\del\varepsilon}{\del T} = \frac{9-p}{4 G_{10}(5-p)} \Omega_{8-p} (r_p r_0)^{(7-p)/2} r_0~.
%\label{eq:}
%
\end{align}
%\end{subequations}
%We consider $p<5$ since the heat capacity diverges for $p=5$ and becomes negative for $p>5$. 
Here, the area law of the black hole entropy is modified as
%比熱は $p=5$ で発散，$p>5$ で負になるので，以下では $p<5$を考える．なお，ディラトンはニュートン定数の働きをすることから（\sect{SUGRA}），エントロピーの面積則は
\be
%
s = \left. e^{-2\phi} \frac{a}{4G_{10}} \right|_{r=r_0}
%\label{eq:}
%
\ee
since the dilaton plays the role of the effective Newton's constant (\sect{SUGRA}).
%となる．
%One can rewrite thermodynamic quantities with gauge theory variables. For example, the energy density is given by
%ゲージ理論の変数で書き直すと，たとえばエネルギー密度は
%\be
%
%\varepsilon \propto (g_\text{YM}^2 N_c)^{(p-3)/(5-p)} N_c^2 T^{2(7-p)/(5-p)}~.
%\label{eq:energy_Dp_app}
%
%\ee

%%------------------
\subsection{RN-AdS black holes}\label{sec:RNAdS}
%%------------------

The RN-AdS$_5$ black hole is given by
%RN-AdS$_5$ブラックホール（プラナー・ホライズン）は
%\be
%
%\action =  \frac{1}{16\pi G_5} \int d^{5}x\, \sqrt{-g} \left(R - 2\Lambda - \frac{L^2}{4}F^2 \right)~.
%\label{eq:}
%
%\ee
%の解であり，
%\mathindent=0zw % <-- [1]
%\begin{subequations}
%\label{eq:}
\begin{align}
%
ds_5^2 &= - f dt^2 + \frac{dr^2}{f} + \left(\frac{r}{L}\right)^2 d\bmx_3^2~, \\
f &= \left(\frac{r}{L}\right)^2 
\left\{ 1 - \left( \frac{\ro}{r} \right)^2 \right\}  
\left\{ 1 - \left( \frac{\ri}{r} \right)^2 \right\}  
\left\{ 1 + \frac{\ro^2+\ri^2}{r^2} \right\}~, \\
% corrected: 2013/9/23
A_0 &= - \frac{\ro}{L^2} \sqrt{3\alpha^2(1+\alpha^2)}
\left(\frac{\ro^2}{r^2} - 1\right)~,
\label{eq:RNAdS_Maxwell}
%
\end{align}
%\end{subequations}
%\mathindent=2zw % <-- [2] デフォルト
($\alpha:=\ri/\ro$). The horizons are located at $r=\ro, \ri$. 
%（$\alpha:=\ri/\ro$）．ホライズンは$r=\ro, \ri$である．熱力学量は，
%We choose the gauge $A_0(r=r_+)=0$ (\sect{other_examples}). 

%We define the chemical potential $\mu$ as $\mu = \left. A_0 \right|_{r=\infty}$ in the text. But a care is necessary because the bulk Maxwell field has the gauge symmetry:
%\begin{subequations}
%\be
%
%A_M(x,r) \to A_M(x,r) - \del_M \Lambda(x,r)~,
%\label{eq:bulk_gauge}
%
%\ee
%or
%\begin{align}
%
%A_\alpha(x,r) &\to A_\alpha(x,r) - \del_\alpha \Lambda(x,r)~, \\
%A_r(x,r) &\to A_r(x,r) - \del_r \Lambda(x,r)~.
%\label{eq:}
%
%\end{align}
%\end{subequations}
%One normally chooses the $A_r=0$ gauge, but the gauge is not completely fixed. There is a residual gauge symmetry
%\be
%
%A_\alpha(x, r) \rightarrow A_\alpha(x, r) + \del_\alpha\Lambda(x)~,
%
%\ee
%so the definition $\mu =  \left. A_0 \right|_{r=\infty}$ is not gauge invariant. There are two options:

%\begin{enumerate}

%\item One can define $\mu$ in a gauge-invariant manner by
%\be
%
%\mu = \left. A_0 \right|_{r=\infty} - \left. A_0 \right|_{r=\ro}~.
%\label{eq:def_chemical1}
%
%\ee
%Namely, what is physical is the difference of the bulk gauge potential between the horizon and the AdS boundary.

%\item Or one can fix the gauge further by requiring
%\be
%
% \left. A_0 \right|_{r=\ro} = 0~.
%\label{eq:}
%
%\ee
%Then, the definition \eqref{eq:def_chemical1} reduces to  $\mu =  \left. A_0 \right|_{r=\infty}$. This definition is normally used and was used in \eq{RNAdS_Maxwell}. 

%\end{enumerate}

Thermodynamic quantities are given by
%\begin{subequations}
%\label{eq:}
\begin{align}
%
T &= \frac{\ro}{2\pi L^2}(2 - \alpha^2 - \alpha^4)~,
\\ %\label{eq:}
\Omega &= - \frac{V_3}{16\pi G_5 L} \left( \frac{\ro}{L} \right)^4 (1 + \alpha^2 + \alpha^4)~,
\\ %\label{eq:}
s &= - \frac{1}{V_3} \left(\frac{\del \Omega}{\del T} \right)_{V_3, \mu}
= \frac{1}{4 G_5}\left(\frac{\ro}{L}\right)^3~,
\\ %\label{eq:}
% corrected: 2013/9/23
\mu &= \left. A_0 \right|_{r\rightarrow\infty} 
= \frac{\ro}{L^2} \sqrt{ 3\alpha^2(1+ \alpha^2) }~,
\\ %\label{eq:}
% corrected: 2013/9/23
\rho &=  - \frac{1}{V_3} \left( \frac{\del \Omega}{\del \mu} \right)_{T, V_3}
= \frac{1}{8\pi G_5} \left( \frac{\ro}{L} \right)^3 \sqrt{ 3\alpha^2(1+ \alpha^2) }~,
\\ %\label{eq:}
\varepsilon &= \frac{\Omega}{V_3} + Ts + \mu\rho 
= \frac{3}{16\pi G_5 L} \left( \frac{\ro}{L} \right)^4 (1 + \alpha^2 + \alpha^4)~,
\\ %\label{eq:}
P &= - \frac{\Omega}{V_3}
= \frac{1}{3} \varepsilon~.
%\label{eq:}
%
\end{align}
%\end{subequations}
To compute thermodynamic quantities, one has to fix, \eg, $\mu$. To do so, rewrite $d\mu=0$ as the condition for $\ro$ and $\alpha$:
\be
%
d\mu = \frac{\del\mu}{\del \ro} d\ro + \frac{\del\mu}{\del \alpha} d\alpha = 0
\result 
d\alpha = - \frac{\alpha(1+\alpha^2)}{1+2\alpha^2} \frac{d\ro}{\ro}~.
%\label{eq:}
%
\ee
Imposing this condition, one gets
\begin{align}
%
d\Omega &= \frac{\del\Omega}{\del \ro} d\ro + \frac{\del\Omega}{\del \alpha} d\alpha 
= - \frac{V_3}{8\pi G_5 L^2} \left( \frac{\ro}{L} \right)^3 (2 + \alpha^2 + \alpha^4) d\ro~,
\\
dT &= \frac{\del T}{\del \ro} d\ro + \frac{\del T}{\del \alpha} d\alpha 
= \frac{1}{2\pi L^2} (2 + \alpha^2 + \alpha^4) d\ro~.
%\label{eq:}
%
\end{align}
Thus,
\be
%
s = - \frac{1}{V_3} \left(\frac{\del \Omega}{\del T} \right)_{V_3, \mu} 
= \frac{1}{4 G_5}\left(\frac{\ro}{L}\right)^3~.
%\label{eq:}
%
\ee

%The RN-AdS \bh is invariant under $x^\mu \rightarrow a x^\mu$, $r \rightarrow r/a$, and $r_\pm \rightarrow r_\pm/a$, so the energy-momentum tensor is traceless. This is similar to the SAdS black hole, but the RN-AdS \bh has an additional dimensionless parameter $\alpha=\ri/\ro$ or $\mu/T$, and the solutions with different $\alpha$ are physically distinct. As a result, not all temperatures are equivalent for the RN-AdS black hole.
%The RN-AdS \bh has the traceless energy-momentum tensor. For the SAdS black hole, the solutions with different horizon radii are all equivalent. As the result of the scale invariance, the \bh has the traceless energy-momentum tensor. The RN-AdS \bh is parametrized by a dimensionless parameter $\alpha$, and the solutions with different $\alpha$ are physically distinct. But the energy-momentum tensor is still traceless. 

Similarly, the RN-AdS$_4$ black hole is given by
%RN-AdS$_4$ブラックホール（プラナー・ホライズン）は
%\mathindent=0zw % <-- [1]
%\begin{subequations}
%\label{eq:}
\begin{align}
%
ds_4^2 &= - f dt^2 + \frac{dr^2}{f} + \left(\frac{r}{L}\right)^2 d\bmx_2^2~, \\
f &= \left(\frac{r}{L}\right)^2
\left( 1 - \frac{\ro}{r} \right)
\left( 1 - \frac{\ri}{r} \right)  
% corrected: 2013/9/23
\left( 1 + \frac{\ro+\ri}{r} + \frac{\ro^2+\ro\ri+\ri^2}{r^2} \right)~, \\
A_0 &= - \frac{2\ro}{L^2} \sqrt{ \alpha(1+\alpha+\alpha^2) }
\left(\frac{\ro}{r}-1\right)~,
%\label{eq:}
%
\end{align}
%\end{subequations}
%\mathindent=2zw % <-- [2] デフォルト
($\alpha:=\ri/\ro$). Thermodynamic quantities are given by
%（$\alpha:=\ri/\ro$）．熱力学量は，
%\begin{subequations}
%\label{eq:}
\begin{align}
%
T &= \frac{\ro}{4\pi L^2}(3 - \alpha - \alpha^2 - \alpha^3)~,
\\ %\label{eq:}
\Omega &= - \frac{V_2}{16\pi G_4 L} \left( \frac{\ro}{L} \right)^3 (1 + \alpha + \alpha^2 + \alpha^3)~,
\\ %\label{eq:}
s &= - \frac{1}{V_2} \left( \frac{\del \Omega}{\del T} \right)_{V_2, \mu}
= \frac{1}{4 G_4}\left(\frac{\ro}{L}\right)^2~,
\\ %\label{eq:}
\mu &= \left. A_0 \right|_{r\rightarrow\infty} 
= \frac{2\ro}{L^2} \sqrt{ \alpha(1+ \alpha+\alpha^2) }~,
\\ 
%\label{eq:} 
\rho &= - \frac{1}{V_2} \left( \frac{\del \Omega}{\del \mu} \right)_{T, V_2}
=  \frac{1}{8\pi G_4} \left( \frac{\ro}{L} \right)^2 \sqrt{ \alpha(1+ \alpha+\alpha^2) }~,
\\ %\label{eq:}
\varepsilon &= \frac{\Omega}{V_2} + Ts + \mu\rho 
= \frac{1}{8\pi G_4 L} \left( \frac{\ro}{L} \right)^3 (1 + \alpha + \alpha^2 + \alpha^3)~,
\\ %\label{eq:}
P &= - \frac{\Omega}{V_2}
= \frac{1}{2} \varepsilon~.
%\label{eq:}
%
\end{align}
%\end{subequations}

%%------------------
\subsection{$d=5$ R-charged black hole and holographic current anomaly}\label{sec:r-charged}
%%------------------

The $d=5$ R-charged black hole is the solution of the five-dimensional $\mathcal{N}=2$ gauged $U(1)^3$ supergravity:
\begin{align}
%
\action 
&=  \frac{1}{16\pi G_5} \int d^{5}x\, \sqrt{-g} \left(R 
 - \frac{L^2}{2}G_{ij} F^i_{MN}F^{MN~j} 
 - G_{ij} \del_M X^i \del^M X^j 
 + \frac{4}{L^2}\, \sum_{i=1}^3 \frac{1}{X^i} \right.
\nonumber \\
  &\hspace*{2.0cm} \left.
 + \frac{L^3}{24\sqrt{-g}}\, \epsilon^{ABCDE}\,\epsilon_{ijk}\,
     F^i_{AB} F^j_{CD} A^k_{E} \right)~.
\label{eq:action_3_charge}
%
\end{align}
%\begin{align}
%   \calL_5
%  &= \sqrt{-g}~\left[~R
%  - \frac{1}{4}\, G_{ij}\, F^i_{\mu\nu}\, F^{j\,\mu\nu}
%  - \frac{1}{2}\, G_{ij}\, \left( \nabla_\mu X^i \right)\,
%                           \left( \nabla^\mu X^j \right)
%  + \frac{4}{L^2}\, \sum_{i=1}^3 \frac{1}{X^i}~\right]
%\nonumber \\
%  &\hspace*{2.0cm}
%  + \frac{1}{24}\, \epsilon^{\mu\nu\rho\sigma\lambda}\,\epsilon_{ijk}\,
%     F^i_{\mu\nu} F^j_{\rho\sigma} A^k_{\lambda}~.
%\label{eq:reduced-action-3charge}
%\end{align}
Here, $F^i_{MN}$ are the field strength of the three $U(1)$ gauge fields $A^i_M$~($i= 1, 2, 3$).
The fields $X^i$~($i=1, 2, 3$) represent three real scalar fields which are not independent but are subject to the constraint $X^1\, X^2\, X^3 = 1$,  and their ``moduli space metric" $G_{ij}$ is given by
\be
%
G_{ij} = \frac{1}{2} \text{diag}[~(X^1)^{-2},\, (X^2)^{-2},\, (X^3)^{-2}~]~.
%
\ee
Note that $\epsilon^{ABCDE}$ is the Levi-Civita symbol not the Levi-Civita tensor: it is purely numerical and takes values $\pm 1$.

The solution is given by
%\begin{subequations}
%\label{eq:}
\begin{align}
%
ds_5^2
  &= - \calH^{-2/3}f dt^2 + \calH^{1/3} f^{-1} dr^2 + \calH^{1/3} \left(\frac{r}{L}\right)^2 d\bmx_3^2~, 
%\quad
%T_0 = \frac{r_+}{\pi L^2}
%\label{eq:}
\\
A_0^i
  &= - \frac{\tilde{\kappa_i}}{L} 
          \left[\left(\frac{r_+}{r}\right)^2\frac{1}{H_i} - \frac{1}{1+\kappa_i} \right]~,
\\ %\label{eq:}
X_i &= \frac{\calH^{1/3}}{H_i}~,
%\label{eq:}
%
\end{align}
where the outer horizon is located at $r=\ro$, and
\begin{align}
H_i &:= 1+ \kappa_i \left(\frac{r_+}{r}\right)^2~, \quad
\calH := H_1 H_2 H_3~, \\
f &:= \left(\frac{r}{L}\right)^2 \left[ \calH - \left(\frac{r_+}{r}\right)^4 \prod_{i=1}^3 (1+\kappa_i) \right]~,
\\ %\label{eq:}
\tilde{\kappa}_i &:= \frac{r_+}{L} \sqrt{\kappa_i} \prod_{l=1}^3 (1+\kappa_l)^{1/2}~.
%\label{eq:}
%
\end{align}
%\end{subequations}
%When $\kappa_i=\kappa$, the solution reduces to the RN-AdS$_5$ black hole. The RN-AdS$_5$ black hole can be written as
%\begin{align}
%
%ds_5^2 &= - f dt^2 + \frac{dr^2}{f} + \left(\frac{r}{L}\right)^2 d\bmx_3^2~, \\
%f &= \left(\frac{r}{L}\right)^2 - \frac{m_\text{RN}}{r^2} + \frac{q_\text{RN}^2}{r^4}~.
%
%\end{align}
%This form is related to the R-charged black hole by a coordinate transformation $r^2+\kappa \ro^2 \rightarrow r^2$ with $m_\text{RN}L^2 = \ro^4(1+\kappa)^3$ and $q_\text{RN}^2 L^2 = \ro^6 \kappa (1+\kappa)^3$.

Thermodynamic quantities are given by%
\footnote{When a metric takes the form
$
ds^2 = - f(r) dt^2 + dr^2/g(r) +\cdots~,
$
the Hawking temperature is given by 
$
T=\sqrt{ f'(r_0)g'(r_0) }/(4\pi)
$
following the derivation in \sect{Euclidean}.
}
%\begin{subequations}
%\label{eq:}
\begin{align}
%
T &= \frac{2 + \kappa_1 + \kappa_2 + \kappa_3 - \kappa_1\kappa_2\kappa_3}
{2\sqrt{(1+\kappa_1)(1+\kappa_2)(1+\kappa_3)}}T_0~, 
\label{eq:temperature} \\
%\displaybreak
s &= \frac{\pi^2 N_c^2 T_0^3}{2}  \prod_{i=1}^3 (1+\kappa_i)^{1/2}~,
\\ %\label{eq:}
%\displaybreak
\mu_i &= \left. A_0^i \right|_{r\rightarrow\infty} 
=\pi T_0 \frac{ \sqrt{\kappa_i} }{1 + \kappa_i} \prod_{l=1}^3 (1+\kappa_l)^{1/2}~, 
\\ %\label{eq:}
\rho_i &= \frac{\pi N_c^2 T_0^3}{4}~\sqrt{\kappa_i} \prod_{l=1}^3 (1+\kappa_l)^{1/2}~,
\\ %\label{eq:}
\varepsilon &= \frac{3 \pi^2 N_c^2 T_0^4}{8} \prod_{i=1}^3 (1+\kappa_i)~, 
\\
P &= \frac{1}{3} \varepsilon~,
%
\end{align}
%\end{subequations}
where $T_0 := r_+/(\pi L^2)$.

%%-------------------------------------
\subsubsection*{Equal-charge case}%\label{sec:}
%%-------------------------------------

The scalar fields are constant $X^i=1$ when $F^i_{MN} = F_{MN}/\sqrt{3}$. Then, the action becomes
\be
%
\action 
=  \frac{1}{16\pi G_5} \int d^{5}x\, \left\{ \sqrt{-g} \left(R + \frac{12}{L^2}
 - \frac{L^2}{4} F_{MN}F^{MN} \right)
 + \frac{L^3}{12\sqrt{3}}\, \epsilon^{ABCDE}\,
     F_{AB} F_{CD} A_{E} \right\}~.
\label{eq:action_equal_charge}
%
\ee
The action \eqref{eq:action_equal_charge} contains the \keyword{Chern-Simons term}. We consider the electric solution, so the Chern-Simons term does not affect the solution. Then, the R-charged black hole reduces to the RN-AdS$_5$ black hole. 

However, the Chern-Simons term has an important consequence. Because the Chern-Simons term explicitly contains the gauge potential $A_E$, the bulk action is not gauge invariant at the AdS boundary. From the boundary point of view, this gives the \keyword{current anomaly}.

The \Nfour\ SYM has the global $SO(6)$ R-symmetry, so the theory has conserved currents. When the SYM is coupled with the external gauge fields for the currents, it is known that the R-symmetry becomes anomalous and the currents are not conserved. In the present case, we pick up a $U(1)$ subgroup of the R-symmetry, and we have a $U(1)$ current. Since we have the bulk Maxwell field, the SYM has the external $U(1)$ gauge field for the current. But the bulk Chern-Simons term spoils the bulk gauge invariance and the current is not conserved as we see below.

The equation of motion for the Maxwell field is given by 
\be
%
\del_N \left(\sqrt{-g} F^{MN} \right) 
+ \frac{L}{4\sqrt{3}} \epsilon^{MABCD}\,F_{AB} F_{CD} = 0~.
\label{eq:Maxwell_CS}
%
\ee
Using the GKP-Witten relation, one can show
\begin{align}
%
\bra J^\mu \ketj 
&= \frac{\delta \Sos}{\delta A_\mu^{(0)}} \\
&= \left. \frac{L^2}{16\pi G_5} \left[ \sqrt{-g} F^{\mu r} 
+ \frac{L}{3\sqrt{3}} \epsilon^{r\mu\nu\rho\sigma}\,A_{\nu}F_{\rho\sigma} \right] \right|_{r\rightarrow\infty}~.
\label{eq:current_dict_CS}
%
\end{align}
The first term is essentially the same as Eqs.~\eqref{eq:response_rho_ads} and \eqref{eq:response_current_ads}. Substituting \eq{current_dict_CS} into the $r$-component of \eq{Maxwell_CS}, one gets
\be
%
\del_\mu \bra J^\mu \ketj 
=  -\frac{1}{16\pi G_5} \frac{L^3}{12\sqrt{3}} \epsilon^{\mu\nu\rho\sigma}\,F_{\mu\nu}F_{\rho\sigma}~,
%\label{eq:}
%
\ee
where $\epsilon^{\mu\nu\rho\sigma}=\epsilon^{r\mu\nu\rho\sigma}$. Thus, the current is not conserved.

See, \eg, Refs.~\cite{Son:2009tf,Nakamura:2009tf} for phenomenological applications of the anomaly.

\endofsection


==> refs/preface_ref.tex <==
\begin{thebibliography}{99}

%
% preface
%

\bibitem{topcites}
%\begin{verbatim} 
\url{https://inspirehep.net/info/hep/stats/topcites/index}
%\end{verbatim} 
%http://www.slac.stanford.edu/spires/topcites/

%\cite{Maldacena:1997re}
\bibitem{Maldacena:1997re}
  J.~M.~Maldacena,
  ``The Large N limit of superconformal field theories and supergravity,''
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 2 } (1998)  231
  [hep-th/9711200].

\end{thebibliography}

